CONFAIR: Configurable and Interpretable Algorithmic Fairness

The rapid growth of data in the recent years has led to the development of complex learning algorithms that are often used to make decisions in real world. While the positive impact of the algorithms has been tremendous, there is a need to mitigate any bias arising from either training samples or implicit assumptions made about the data samples. This need becomes critical when algorithms are used in automated decision making systems that can hugely impact people's lives. Many approaches have been proposed to make learning algorithms fair by detecting and mitigating bias in different stages of optimization. However, due to a lack of a universal definition of fairness, these algorithms optimize for a particular interpretation of fairness which makes them limited for real world use. Moreover, an underlying assumption that is common to all algorithms is the apparent equivalence of achieving fairness and removing bias. In other words, there is no user defined criteria that can be incorporated into the optimization procedure for producing a fair algorithm. Motivated by these shortcomings of existing methods, we propose the CONFAIR procedure that produces a fair algorithm by incorporating user constraints into the optimization procedure. Furthermore, we make the process interpretable by estimating the most predictive features from data. We demonstrate the efficacy of our approach on several real world datasets using different fairness criteria.

==> figures/comparison_fig.tex <==
\begin{figure*}[t]
    \centering
    \subfigure[]{\includegraphics[width=\columnwidth]{figures/adult_ftol_analysis.pdf}}\\
    \subfigure[]{\includegraphics[width=\columnwidth]{figures/compas_ftol_analysis_missing_fairlearn.pdf}}\\
    \subfigure[]{\includegraphics[width=\columnwidth]{figures/german_data_plot.pdf}}
    \caption{Caption}
    \label{fig:ftol_effect}
\end{figure*}


==> preface.tex <==
% This section allows us to modify preloaded package properties
\makeatletter
% These magic runes make comment's appear inline
% These also need to be above the other magic runes
\usepackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}
\usepackage{regexpatch}
\xpatchcmd{\@todo}{\setkeys{todonotes}{#1}}{\setkeys{todonotes}{inline,#1}}{}{}

% These magic runes make the new changes package work with comments
\usepackage{comment}
\let\wfs@comment@comment\comment
\let\comment\@undefined
\usepackage{changes}
\let\wfs@changes@comment\comment
\let\comment\@undefined
\newcommand\comment{%
    \ifthenelse{\equal{\@currenvir}{comment}}
    {\wfs@comment@comment}
    {\wfs@changes@comment}%
}
\makeatother

% Typical preloader time

\usepackage{hyperref}
\usepackage{enumitem}
\usepackage{multirow}
\usepackage{outlines}
\usepackage{graphicx}
\usepackage{algorithm}
\usepackage{float}
\usepackage{nicefrac}
\usepackage{url}
% \usepackage{booktabs}
\usepackage{listings}
\usepackage{todonotes}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{subfigure}
\lstset{
  basicstyle=\ttfamily,
  columns=fullflexible,
  frame=single,
  breaklines=true,
  tabsize=2,
  breakautoindent=true,
}
% nt -> env, disp text, [counter reset follow]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem{proposition}{Proposition}[section]
% Changes Authors
\definechangesauthor[name="Ankit Kulshrestha", color=blue]{ak}
% \definechangesauthor[name="Ilya Tyagin", color=cyan]{it}
% \definechangesauthor[name="Justin Sybrandt", color=green]{js}
\definechangesauthor[name="Ilya Safro", color=red]{is}


\newcommand{\pymoliererepo}{
% \href{http://sybrandt.com/2020/agatha}
% {sybrandt.com/2020/agatha}
}
\newcommand{\pymoliere}{AGATHA}

% These are shortcuts for leaving specific changes comments
\newcommand{\note}[2]{\added[id=#1, comment={#2}]{}}

% Ankit's add, delete, replace
\newcommand{\Aak}[1]{\added[id=ak]{#1}}
\newcommand{\Dak}[1]{\deleted[id=ak]{#1}}
\newcommand{\Rak}[2]{\replaced[id=ak]{#1}{#2}}

% Justin's add, delete, replace
\newcommand{\Ajs}[1]{\added[id=js]{#1}}
\newcommand{\Djs}[1]{\deleted[id=js]{#1}}
\newcommand{\Rjs}[2]{\replaced[id=js]{#1}{#2}}

% ITyagin's add, delete replace
\newcommand{\Ait}[1]{\added[id=it]{#1}}
\newcommand{\Dit}[1]{\deleted[id=it]{#1}}
\newcommand{\Rit}[2]{\replaced[id=it]{#1}{#2}}

% ISafro's add, delete, replace
\newcommand{\Ais}[1]{\added[id=is]{#1}}
\newcommand{\Dis}[1]{\deleted[id=is]{#1}}
\newcommand{\Ris}[2]{\replaced[id=is]{#1}{#2}}

% THIS ALLOWS FOR CONDITIONAL COMMENTS
% \newif\ifthesis
% Comment/ un-comment as needed
% \thesisfalse
%\thesistrue

% Comment out a block of text for KDD (but keep for thesis) with this syntax:
% \ifthesis
% <Text to comment out>
% \else [Optional]
% <Optional replacement for KDD Version>
% \fi

\hyphenation{
    AG-A-THA
}

% These magic runes make everything denser
\setlength{\textfloatsep}{3pt}
\setlength{\floatsep}{3pt}
\setlength{\belowdisplayskip}{3pt} \setlength{\belowdisplayshortskip}{3pt}
\setlength{\abovedisplayskip}{3pt} \setlength{\abovedisplayshortskip}{3pt}

% \settopmatter{authorsperrow=4}

% \newcommand{\sysnameo}{AGATHA-O }
% \newcommand{\sysnamec}{AGATHA-C }
% \newcommand{\sysnamegp}{AGATHA-GP }

\usepackage{mathtools}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}


==> tables/baseline_fairlearn_backup.tex <==
\begin{table*}[htbp]
    \centering
    \small
    \setlength{\tabcolsep}{1pt}
    \begin{center}
    \begin{tabular}{l|ccc|ccc|ccc}
      \hline\hline
       Method   & 
       \multicolumn{3}{c}{GERMAN} &
       \multicolumn{3}{c}{COMPAS} & 
       \multicolumn{3}{c}{ADULT} &\\
    %   \cmidrule(lr){2-5}
    %   \cmidrule(lr){6-9}
    %   \cmidrule(lr){10-13}
    %   \cmidrule(lr){14-17}
    %     % \cline{2-5}
        % \cline{6-9}
        % \cline{10-13}
        % \cline{14-17}
      
 
       {} & 
       $f_{\text{tol}}$ & Acc. & DEO & NPV &
       $f_{\text{tol}}$ & Acc. & DEO & NPV &
       $f_{\text{tol}}$ & Acc. & DEO & NPV  \\
      \hline 
      
      SVM  & $0.76\pm0.06$ & $0.04 \pm 0.02$ & $0.08 \pm 0.04$ & - & $0.67 \pm 0.02$ & $0.30 \pm 0.08$ & $0.06 \pm 0.03$ & - & $0.83$ & $0.129$ & $0.10$ & - &  \\
      
      FairSVM  & $1e^{-3}$ & $0.75 \pm 0.01$ & $0.04 \pm 0.02$ & $0.08 \pm 0.04$ &  $0$ & $0.67 \pm 0.005$ & $0.28 \pm 0.04$ & $0.023 \pm 0.007$ & $1e^{-1}$ & $0.824$ & $0.081$ & $0.10$ & \\
      
      
      FAIRLEARN-SVM  & $1e^{-3}$ & $\textbf{0.74} \pm 0.04$ & $\textbf{0.024} \pm 0.01$ & $0.12 \pm 0.07$ & $0$ & $0.68 \pm 0.006$ & $\textbf{0.15} \pm 0.023$ & $\textbf{0.01} \pm 0.01$ & $1e^{-1}$ & $\textbf{0.831}$ & $\textbf{0.009}$ & $0.1268$ & - & $0.92 \pm 0.001$ & $0.59 \pm 0.06$ & $0.02 \pm 0.01$ \\
      
      \midrule
      \midrule
      
      Lin. SVM & - & $0.76 \pm 0.06$ & $0.04 \pm 0.02$ & $0.08 \pm 0.04$ & - & $0.67 \pm 0.02$ & $0.30 \pm 0.08$ & $0.06 \pm 0.03$ & - & $0.83$ & $0.129$ & $0.10$ & - & $0.92 \pm 0.001$ & $0.59 \pm 0.06$ & $0.02 \pm 0.01$ \\
      
      
      Lin. FairSVM  & - & $0.76 \pm 0.06$ & $0.04 \pm 0.02$ & $0.08 \pm 0.04$ & - & $0.67 \pm 0.02$ & $0.30 \pm 0.08$ & $0.06 \pm 0.03$ & - & $0.83$ & $0.129$ & $0.10$ & - & $0.92 \pm 0.001$ & $0.59 \pm 0.06$ & $0.02 \pm 0.01$ \\
      
      Lin. FAIRLEARN-SVM  & - & $0.76 \pm 0.06$ & $0.04 \pm 0.02$ & $0.08 \pm 0.04$ & - & $0.67 \pm 0.02$ & $0.30 \pm 0.08$ & $0.06 \pm 0.03$ & - & $0.83$ & $0.129$ & $0.10$ & - & $0.92 \pm 0.001$ & $0.59 \pm 0.06$ & $0.02 \pm 0.01$ \\
      
      
    %   Lin. FairSVM & 
      
    %   \hline
      
      \bottomrule
      
    \end{tabular}    
    \end{center}
    
    
    \caption{Comparison of FAIRLEARN SVM with two baseline methods - unfair SVM and a fair SVM trained with all features equally weighted.}
    \label{tab:backup_main}
\end{table*}

==> tables/comparison_table.tex <==
\begin{table}[htbp]
    \centering
    \begin{tabular}{l|cc|cc|cc}
      \hline\hline 
       Method &  
       \multicolumn{2}{c|}{GERMAN} & 
       \multicolumn{2}{c|}{ADULT} & 
       \multicolumn{2}{c}{COMPAS}\\
       \hline
         & Acc & DEO & Acc & DEO & Acc & DEO\\
        \hline
        Lin. FairSVM & & & & & \\[.5ex]
        Lin. FAIRLEARN & & & & & \\[.5ex]
        Hardt.~\emph{et al.} & & & & & \\[.5ex]
        Zafar \emph{et al.} & & & & & \\[.5ex]
        Lin. FERM  & & & & & \\[.5ex]
        \hline\hline
        FairSVM & & & & & \\[.5ex]
        FAIRLEARN & & & & & \\[.5ex]
        Hardt.~\emph{et al.} & & & & & \\[.5ex] 
        FERM & & & & &
    \end{tabular}
    \caption{Comparison of FAIRLEARN against existing fairness methods}
    \label{tab:comparison}
\end{table}

==> tables/crit_feat_description.tex <==
\begin{table}[htbp]
    \centering
    \begin{tabular}{c|c|p{.5\linewidth}}
    \hline\hline
      DATASET & $s \in \mathcal{C}$ & Critical Features\\
      \hline 
       ADULT  & Yes & \\[1.2ex]
      COMPAS & Yes &  Race, Age, Sex, Priors Count \\[1.2ex] 
       GERMAN & &  
    \end{tabular}
    \caption{Critical features found by the FAIRLEARN algorithm.}
    \label{tab:crit_feats}
\end{table}

==> tables/data_sampling_results.tex <==
\begin{table}[ht]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
        Model &  \multicolumn{2}{c}{Drug} & \multicolumn{2}{c}{Arrhythmia} \\
        \cmidrule(lr){2-3}
        \cmidrule(lr){4-5}
         &  Precision & DFPR & Precision & DFPR\\
    \midrule
        SVM  &  $0.672 \pm 0.028$ & $0.12 \pm 0.087$ & $0.744 \pm 0.05$  & $0.251 \pm 0.135$ \\ 
        SVM-MT &  $0.661 \pm 0.032$ & $0.074 \pm 0.04 $& $0.703 \pm 0.03$ & $0.09 \pm 0.06$\\ 
        FERM  & $0.648\pm 0.017$& $0.102 \pm 0.05$& $0.735 \pm 0.03$ & $0.121 \pm 0.07$\\ 
    \bottomrule
    \end{tabular}
    }
    \caption{Results of experiments with undersampling the majority label class on Drug and Arrhythmia datasets. The results are an average of 5 different runs.}
    \label{tab:sampling_expts}
\end{table}

==> tables/dataset_results.tex <==
\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{.3em}
    \begin{tabular}{lcccccccc}
    \toprule
     Method   & 
    \multicolumn{2}{c}{Adult} & 
    \multicolumn{2}{c}{COMPAS} & 
    \multicolumn{2}{c}{Drug} & 
    \multicolumn{2}{c}{Arrhythmia}\\
    \cmidrule(lr){2-3}
    \cmidrule(lr){4-5}
    \cmidrule(lr){6-7}
    \cmidrule(lr){8-9}
    {} & 
    Precision & DFPR &
    Precision & DFPR &
    Precision & DFPR &
    Precision & DFPR \\
    \midrule
    SVM  & 0.74 & 0.086 & $0.668 \pm 0.009$ & $\textbf{0.217}\pm 0.058$ & $0.672 \pm 0.027$ & $0.098 \pm 0.066$ & $0.747 \pm 0.061$ & $\textit{0.158} \pm 0.103$ \\ 
    SVM-MT & 0.73 &  \textbf{0.020} & $0.664 \pm 0.023$ & $\textit{0.225} \pm 0.058$ & $0.625 \pm 0.017$ & $\textbf{0.033} \pm 0.026$ & $0.703 \pm 0.072$ &  $\textbf{0.056} \pm 0.04$ \\ 
    FERM  & 0.71 & \textit{0.067} & $0.667 \pm 0.015$ & $0.25 \pm 0.053$ & $0.627 \pm 0.023$& $\textit{0.069} \pm 0.078$ & $0.742 \pm 0.048$ & $0.21 \pm 0.124$ \\
    \end{tabular}
    \caption{A comparison of results on four datasets with baseline FERM method and optimizing for minimal separation. Best results are shown in bold and second best are in italics.}
    \label{tab:results_main}
\end{table*}


%% Adult COMPAS Drug Arrhythmia

==> tables/timing_results.tex <==
\begin{table}[h]
    \centering
    %\resizebox{\columnwidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
        Model & Adult & COMPAS & Drug & Arrhythmia \\
    \midrule
        SVM &  $1 \pm 1.5$ & $3 \pm 1$ & $1\pm 1$ & $0.2 \pm 0.5$ \\ 
        SVM-MT & $7 \pm 1 $ & $121\pm 1$ & $10\pm 1$& $1\pm0.6$ \\ 
        FERM & $10 \pm 1$ & $136\pm 1$& $16\pm 1$& $2 \pm	1$ \\ 
    \bottomrule
    \end{tabular}
    %}
    \caption{Model optimization times on different datasets. The results are an average of 5 different runs. All times except for Adult dataset are in seconds.  Adult dataset time is measured in minutes.}
    \label{tab:timing_results}
\end{table}
